Holistic Autonomous Driving Understanding by Bird's-Eye-View Injected Multi-Modal Large Models

The rise of multimodal large language models (MLLMs) has spurred interest in language-based driving tasks. However, existing research typically focuses on limited tasks and often omits key multi-view and temporal information which is crucial for robust autonomous driving. To bridge these gaps, we introduce NuInstruct, a novel dataset with 91K multi-view video-QA pairs across 17 subtasks, where each task demands holistic information (e.g., temporal, multi-view, and spatial), significantly elevating the challenge level. To obtain NuInstruct, we propose a novel SQL-based method to generate instruction-response pairs automatically, which is inspired by the driving logical progression of humans. We further present BEV-InMLLM, an end-to-end method for efficiently deriving instruction-aware Bird's-Eye-View (BEV) features, language-aligned for large language models. BEV-InMLLM integrates multi-view, spatial awareness, and temporal semantics to enhance MLLMs' capabilities on NuInstruct tasks. Moreover, our proposed BEV injection module is a plug-and-play method for existing MLLMs. Our experiments on NuInstruct demonstrate that BEV-InMLLM significantly outperforms existing MLLMs, e.g. around 9% improvement on various tasks. We plan to release our NuInstruct for future research development.

==> files/suppexperiment.tex <==

\noindent\textbf{Step 1 - Filter \& Construction.} Given a keyframe with annotations from NuScenes (Fig.~\ref{fig:datageneration}~(a)), we first compute the distances of all instances away from the ego car. Then we regard objects within $20$ meters from the ego car as important instances, while filtering others.
%
Based on the information of the ego car and important instances, we construct a scene information database as shown in Fig.~\ref{fig:datageneration}~(b).
%
The scene information database includes four tables:
\begin{itemize}
    \item \texttt{Scene Information}: consists of the scene dictionary list. The key for each dictionary is the scene ID, which is the unique identifier of the scene in NuScenes~\cite{caesar2020nuscenes}. The value is a frame ID list, consisting of IDs of frames in the current scene. The details for each frame are referred to the \texttt{Frame Information} table.
    %
     \item \texttt{Frame Information}: consists of the frame dictionary list. The key for each dictionary is the unique ID for a specific frame. The value contains the details for the frame, including the ego-car-information ID and instance-information ID list. The details for the information of the ego car and instances in the frame are referred to the \texttt{Ego Information} and \texttt{Instance Information} tables respectively.
     %
    \item \texttt{Ego Information}: consists of the ego-car information dictionary list. The key for each dictionary is the unique ID for the information of the ego-car in one specific frame. The values include the information: ~\eg, ego car pose, ego car rotation, velocity, road information, camera information, and so on. 
    \item \texttt{Instance Information}: consists of the instance information dictionary list. The key for each dictionary is the unique ID for the information of one instance in one specific frame. The values include the information: ~\eg, instance ID (the unique identifier for one instance,~\eg, a car, across different frames in one scene), instance global and local translations and rotations, velocity, road information, etc. 
\end{itemize}
The relations between different tables in the database are shown in Fig.~\ref{fig:datageneration}~(b) (\textcolor{blue}{blue dashed arrows}),~\ie, \texttt{Scene Information} and \texttt{Frame Information}, \texttt{Frame Information} and \texttt{Ego Information}, \texttt{Frame Information} and \texttt{Instance Information} are all one-to-many mappings.
%
Please refer to the supplementary material for more details about the scene information database.
%
% The scene information database is then used for the \textbf{Step 3} to retrieve the response based on the specific task SQLs. 

%---------------
\vspace{0.5mm}
\noindent\textbf{Step 2 - Sampling.} After obtaining the scene information database, we randomly sample three keyframes from one scene in the original dataset, which is then input to a specific task SQL sampled from a series of pre-defined task SQLs.
%
As shown in Fig.~\ref{fig:datageneration}~(c), we define four types of SQL sets (\ie, perception, prediction, risk, and planning with reasoning), which are later used for generating different types of instruction-response pairs.
%
Each type of task SQL set consists of several subtask SQLs.
%
For example, the perception SQL set contains six subtask SQLs,~\eg, Closest focuses on finding the objects closest to the ego car, and the others are similar. \hjh{the others subtasks are similar?}
%
Note that some high-level SQLs may be inherited from low-level ones following the relational flow of autonomous driving tasks~\cite{hu2023planning}, as shown in \textcolor{red}{red dashed arrows} in Fig.~\ref{fig:datageneration}~(c).
%
For instance, the prediction SQLs are based on the perception ones, the risk SQLs are based on both prediction and perception SQLs, and the planning with reasoning SQL is inherited from prediction and risk ones.
%
Please refer to the supplementary material for more details about task SQLs. \hjh{redundant, similar to the last sentence}

\vspace{0.5mm}
\noindent\textbf{Step 3 - Retrieval.}
%
Given the sampled keyframes with annotations, we successively select subtask SQLs,~\eg, the closest subtask from perception SQLs (see Fig.~\ref{fig:datageneration}~(c)). 
%
Each subtask consists of a subtask function and an instruction prompt.
%
Receiving the informations of an instance or the ego car as input, the subtask function retrieves the responses from the scene information database (see Fig.~\ref{fig:datageneration}~(b)).
%
We also show some \hjh{more detailed} examples in Fig.~\ref{fig:example}. \hjh{step2 and 3}


\noindent\textbf{Step 4 - Saving.}
%
After obtaining the instruction prompts and their corresponding responses from \textbf{Step 3}, we save all different instruction-response pairs for different tasks.
%
Furthermore, we employ GPT-4~\cite{OpenAI_2023} to revise the responses for more fluent and reasonable.

We only describe the overview of the data generation in this section.
Please refer to the supplementary material for more details about the scene information database, the task SQLs, and the retrieval process.

% \begin{table}
% \centering
% \caption{ \textbf{Evaluation metrics for different tasks.} $\downarrow$ represents the lower the scores, the better the results, while $\uparrow$ means the higher the scores, the better the results. `MAE' indicates the mean absolute error. `All' means the all subtasks.
% %
% \vspace{-1.0em}}
% % \begin{footnotesize}
% \resizebox{0.7\columnwidth}{!}{
%   % \begin{adjustbox}{max width=0.8\linewidth}
%   \begin{tabular}{c|l|l}
%     % \toprule
%     \Xhline{1.0pt}
%   Task & SubTask & Metrics \\
% %      % \cmidrule{3-6} \cmidrule{8-8} 
% %     \\
%      % \cmidrule{1-11}
%      \hline
%      % \midrule
% % %     % \cmidrule{1-2} \cmidrule{3-6} \cmidrule{6-11}
%  \multirow{4}{*}{Spatial}   & Distance &  \multirow{2}{*}{MAE $\downarrow$}  \\
%    % & MiniGPT-4 & \\
%   & Motion\\
%    \cline{2-3}
%    & Status &  \multirow{2}{*}{Accuracy $\uparrow$}\\
%    & Closest \\
%   \hline
%    \multirow{3}{*}{Temporal} & Speed & \multirow{2}{*}{MAE $\downarrow$} \\
%    % & MiniGPT-4 & \
%      & Motion \\
%   & status & Accuracy $\uparrow$  \\
 
% \hline
% \multirow{2}{*}{Multi-view}& Instance number &  MAP $\uparrow$\\
%  & Same Road \\
% \hline
%    \multirow{2}{*}{Whole} & Risk \\
%       & Planning \\
% % \bottomrule
% % {\multicolumn{2}{c|}{Risk}}  & MAP $\uparrow$ \\
% \hline
% % {\multicolumn{2}{c|}{Reasoning}}  & Bleu $\uparrow$ \\
% % \hline
%     \end{tabular}
%     % \end{adjustbox}
%     }
%     \label{tab:categorytask}
% % \end{footnotesize}
% \end{table}


\definecolor{mygreen}{rgb}{0.0, 0.51, 0.0}
\definecolor{color1}{rgb}{0.98, 0.81, 0.69}


% \begin{table}
%     \centering
%     \caption{The ablation study of different proposed modules.  \textbf{(a)} The base model MiniGPT-4~\cite{zhu2023minigpt}. \textbf{(b)} The base model with ST-Adapter to capture the temporal cues. \textbf{(c)} MV-MLLM (Section~\ref{sec:baseline}) enhancing (b) with MV information. \textbf{(d)} Incorporating BEV into (b) for spatial cues. \textbf{(e)} BEV-InMLLM (Section~\ref{sec:bev-inmllm}) capturing all informations.}
%     \vspace{-3.0mm}
%     \label{tab:rgr_with_and_without_artifacts}
%     \begin{adjustbox}{max width=\linewidth}
%     \begin{tabular}{c|ccc|cc|cc|cc|c}
%     \Xhline{1.5pt}
%     \rowcolor{mygray}
%     &
%     &
%     &
%     &\multicolumn{2}{c|}{\small  \it \textbf{Temporal}}
%     &\multicolumn{2}{c|}{\small  \it \textbf{Multi-view}}
%     &\multicolumn{2}{c|}{\small  \it \textbf{Spatial}}
%     &
%     \\
%     \rowcolor{mygray}
%      \multirow{-2}{*}{\small \textbf{Model}}
%     &\multirow{-2}{*}{\small  \textbf{T}} 
%     &\multirow{-2}{*}{\small  \textbf{MV}}
%     &\multirow{-2}{*}{\small  \textbf{BEV}}
%     &\textbf{$\downarrow$}
%     &\textbf{$\uparrow$}
%      &\textbf{$\downarrow$}
%     &\textbf{$\uparrow$}
%    &\textbf{$\downarrow$}
%     &\textbf{$\uparrow$}
%     & \multirow{-2}{*}{\small \it \textbf{Whole} $\uparrow$}\\
%     % \cmidrule{1-1} \cmidrule{3-3} \cmidrule{5-5} \cmidrule{7-9} \cmidrule{11-15}
%   \midrule
%     \textbf{(a)}  & \XSolidBrush & \XSolidBrush  &  \XSolidBrush & 10.3 & 25.8 & 6.7 & 22.7 & 20.8 & 27.6 & 12.4  \\
%     \midrule
%  \multirow{2}{*}{\textbf{(b)}}  & \multirow{2}{*}{\Checkmark} &  \multirow{2}{*}{\XSolidBrush}  &  \multirow{2}{*}{\XSolidBrush} &  7.4 \textbf{\textcolor{mygreen}{+ 3.9}} & 28.5 &6.3 & 24.2 & 19.5 & 25.7 & 15.7 \\
%  & & & & \textbf{\textcolor{mygreen}{+ 3.9}}& \\
%  \midrule
%      \textbf{(c)}  &\Checkmark& \Checkmark &  \XSolidBrush &  6.4 & 31.4 & 4.1 & 30.7 & 18.0 &30.0 & 20.1\\
%      \textbf{(d)} & \Checkmark & \XSolidBrush  &  \Checkmark & 5.9 & 31.2 & 6.0 & 28.3 & 14.4 & 32.5 & 21.6  \\
%      \midrule
%      \textbf{(e)}  & \Checkmark & \Checkmark &  \Checkmark & 3.7 & 32.8 & 3.8 & 31.5 &13.9&32.9 & 22.2  \\
%   \bottomrule
%     % \multirow{2}{*}{$\times 2$} &\XSolidBrush    &28.16 &0.728 &28.08 &0.702 \\
%     %                             &\Checkmark   &27.99 &0.725 &28.05 &0.692 \\

%     % \midrule
%     % \multirow{2}{*}{$\times 3$} &\XSolidBrush     &27.99 &0.732 &28.42 &0.711 \\
%     %                             &\Checkmark   &27.83 &0.726 &28.47 &0.705 \\
%     % \midrule
%     % \multirow{2}{*}{$\times 4$} &\XSolidBrush    &27.99 &0.730 &28.30 &0.704 \\
%     %                             &\Checkmark   &27.83 &0.729 &28.48 &0.702 \\
%     % \Xhline{1.5pt}
%     \end{tabular}
%     \end{adjustbox}
% % \end{footnotesize}
% \vspace{-1.0em}
% \end{table}

% \begin{table}
%     \centering
%     \caption{The ablation study of different proposed modules.
%     %
%     \textbf{(a)} The full model,~\ie, BEV-InMLLM introduced in Section~\ref{sec:bev-inmllm}.  \textbf{(b)} BEV-InMLLM without temporal cues,~\ie, the input is image.
%     \textbf{(c)} BEV-InMLLM without multi-view information,~\ie, only single-view input.
%     \textbf{(d)} BEV-InMLLM without BEV information,~\ie, without BEV injection module.
%     \textbf{(e)} The baseline model,~\ie, MiniGPT-4~\cite{zhu2023minigpt}.
%     }
%     \vspace{-3.0mm}
%     \label{tab:rgr_with_and_without_artifacts}
%     \begin{adjustbox}{max width=\linewidth}
%     \begin{tabular}{l|cc|cc|cc|c}
%     \Xhline{1.5pt}
%     \rowcolor{mygray}
%     &\multicolumn{2}{c|}{\small  \it \textbf{Temporal}}
%     &\multicolumn{2}{c|}{\small  \it \textbf{Multi-view}}
%     &\multicolumn{2}{c|}{\small  \it \textbf{Spatial}}
%     &
%     \\
%     \rowcolor{mygray}
%      \multirow{-2}{*}{\small \textbf{Model}}
%     &\textbf{$\downarrow$}
%     &\textbf{$\uparrow$}
%      &\textbf{$\downarrow$}
%     &\textbf{$\uparrow$}
%    &\textbf{$\downarrow$}
%     &\textbf{$\uparrow$}
%     & \multirow{-2}{*}{\small \it \textbf{Whole} $\uparrow$}\\
%     % \cmidrule{1-1} \cmidrule{3-3} \cmidrule{5-5} \cmidrule{7-9} \cmidrule{11-15}
%   \midrule
%     (a) Full  & 3.7 & 32.8 & 3.8 & 31.5 &13.9&32.9 & 22.2  \\
%     \midrule
%     (b) - T & 7.4 & 28.5 & 6.3 & 24.2 & 19.5 & 25.7 & 15.7 \\
% & \textbf{\textcolor{mygreen}{+3.7}} & \textbf{\textcolor{mygreen}{+4.3}} & \textbf{\textcolor{mygreen}{+2.5}} & \textbf{\textcolor{mygreen}{+7.3}} & \textbf{\textcolor{mygreen}{+5.6}} & \textbf{\textcolor{mygreen}{+7.2}} & \textbf{\textcolor{mygreen}{+6.5}} \\
%     (c) - MV &  5.9 & 31.2 & 6.0 & 28.3 & 14.4 & 32.5 & 21.6  \\
%     (d) - BEV &   6.4 & 31.4 & 4.1 & 30.7 & 18.0 &30.0 & 20.1\\
%     \midrule
%     (e) Base & 10.3 & 25.8 & 6.7 & 22.7 & 20.8 & 27.6 & 12.4  \\
%   \bottomrule
%     \end{tabular}
%     \end{adjustbox}
% % \end{footnotesize}
% \vspace{-1.0em}
% \end{table}

% \textbf{(c)} - MV & 5.9 (\textbf{\textcolor{mygreen}{+2.2}}) & 31.2 (\textbf{\textcolor{mygreen}{+1.6}}) & 6.0 (\textbf{\textcolor{mygreen}{+2.2}}) & 28.3 (\textbf{\textcolor{mygreen}{+3.2}}) & 14.4 (\textbf{\textcolor{mygreen}{+0.5}}) & 32.5 (\textbf{\textcolor{mygreen}{+0.4}}) & 21.6 (\textbf{\textcolor{mygreen}{+0.6}}) \\
% \textbf{(d)} - BEV & 6.4 (\textbf{\textcolor{mygreen}{+2.7}}) & 31.4 (\textbf{\textcolor{mygreen}{+1.4}}) & 4.1 (\textbf{\textcolor{mygreen}{+0.3}}) & 30.7 (\textbf{\textcolor{mygreen}{+0.8}}) & 18.0 (\textbf{\textcolor{mygreen}{+4.1}}) & 30.0 (\textbf{\textcolor{mygreen}{+2.9}}) & 20.1 (\textbf{\textcolor{mygreen}{+2.1}}) \\
% \textbf{(e)} - Base & 10.3 (\textbf{\textcolor{mygreen}{+6.6}}) & 25.8 (\textbf{\textcolor{mygreen}{+7.0}}) & 6.7 (\textbf{\textcolor{mygreen}{+2.9}}) & 22.7 (\textbf{\textcolor{mygreen}{+8.8}}) & 20.8 (\textbf{\textcolor{mygreen}{+6.9}}) & 27.6 (\textbf{\textcolor{mygreen}{+5.3}}) & 12.4 (\textbf{\textcolor{mygreen}{+9.8}}) \\


% \begin{table}
%     \centering
%     \caption{The ablation study of different proposed modules.  \textbf{(a)} The base model MiniGPT-4~\cite{zhu2023minigpt}. \textbf{(b)} The base model with ST-Adapter to capture the temporal cues. \textbf{(c)} MV-MLLM (Section~\ref{sec:baseline}) enhancing (b) with MV information. \textbf{(d)} Incorporating BEV into (b) for spatial cues. \textbf{(e)} BEV-InMLLM (Section~\ref{sec:bev-inmllm}) capturing all informations.}
%     \vspace{-3.0mm}
%     \label{tab:rgr_with_and_without_artifacts}
%     \begin{adjustbox}{max width=\linewidth}
%     \begin{tabular}{c|ccc|cc|cc|cc|c}
%     \Xhline{1.5pt}
%     \rowcolor{mygray}
%     &
%     &
%     &
%     &\multicolumn{2}{c|}{\small  \it \textbf{Temporal}}
%     &\multicolumn{2}{c|}{\small  \it \textbf{Multi-view}}
%     &\multicolumn{2}{c|}{\small  \it \textbf{Spatial}}
%     &
%     \\
%     \rowcolor{mygray}
%      \multirow{-2}{*}{\small \textbf{Model}}
%     &\multirow{-2}{*}{\small  \textbf{T}} 
%     &\multirow{-2}{*}{\small  \textbf{MV}}
%     &\multirow{-2}{*}{\small  \textbf{BEV}}
%     &\textbf{$\downarrow$}
%     &\textbf{$\uparrow$}
%      &\textbf{$\downarrow$}
%     &\textbf{$\uparrow$}
%    &\textbf{$\downarrow$}
%     &\textbf{$\uparrow$}
%     & \multirow{-2}{*}{\small \it \textbf{Whole} $\uparrow$}\\
%     % \cmidrule{1-1} \cmidrule{3-3} \cmidrule{5-5} \cmidrule{7-9} \cmidrule{11-15}
%   \midrule
%     \textbf{(a)}  & \XSolidBrush & \XSolidBrush  &  \XSolidBrush & 10.3 & 25.8 & 6.7 & 22.7 & 20.8 & 27.6 & 12.4  \\
%     \midrule
%  \multirow{2}{*}{\textbf{(b)}}  & \multirow{2}{*}{\Checkmark} &  \multirow{2}{*}{\XSolidBrush}  &  \multirow{2}{*}{\XSolidBrush} &  7.4& 28.5 &6.3 & 24.2 & 19.5 & 25.7 & 15.7 \\
%  & & & & \textbf{\textcolor{mygreen}{+2.9}} & \textbf{\textcolor{mygreen}{+2.7}} & \textbf{\textcolor{mygreen}{+0.4}} \\
%  \midrule
%      \textbf{(c)}  &\Checkmark& \Checkmark &  \XSolidBrush &  6.4 & 31.4 & 4.1 & 30.7 & 18.0 &30.0 & 20.1\\
%      & & & & \textbf{\textcolor{mygreen}{+1.0}} & \textbf{\textcolor{mygreen}{+2.9}} & \textbf{\textcolor{mygreen}{+2.2}} & \textbf{\textcolor{mygreen}{+6.5}} & \textbf{\textcolor{mygreen}{+1.5}} & \textbf{\textcolor{mygreen}{+4.3}} & \textbf{\textcolor{mygreen}{+4.4}} \\
%      \midrule
%      \textbf{(d)} & \Checkmark & \XSolidBrush  &  \Checkmark & 5.9 & 31.2 & 6.0 & 28.3 & 14.4 & 32.5 & 21.6  \\
%      & & & & \textbf{\textcolor{mygreen}{+0.5}} & \textbf{\textcolor{mygreen}{+0.2}} & \textbf{\textcolor{mygreen}{+1.9}} & \textbf{\textcolor{mygreen}{+2.4}} & \textbf{\textcolor{mygreen}{+3.6}} & \textbf{\textcolor{mygreen}{+2.5}} & \textbf{\textcolor{mygreen}{+1.5}} \\
%      \midrule
%      \textbf{(e)}  & \Checkmark & \Checkmark &  \Checkmark & 3.7 & 32.8 & 3.8 & 31.5 &13.9&32.9 & 22.2  \\
%      & & & & \textbf{\textcolor{mygreen}{+2.2}} & \textbf{\textcolor{mygreen}{+1.6}} & \textbf{\textcolor{mygreen}{+2.2}} & \textbf{\textcolor{mygreen}{+3.2}} & \textbf{\textcolor{mygreen}{+0.5}} & \textbf{\textcolor{mygreen}{+0.4}} & \textbf{\textcolor{mygreen}{+0.6}} \\
%   \bottomrule
%     % \multirow{2}{*}{$\times 2$} &\XSolidBrush    &28.16 &0.728 &28.08 &0.702 \\
%     %                             &\Checkmark   &27.99 &0.725 &28.05 &0.692 \\

%     % \midrule
%     % \multirow{2}{*}{$\times 3$} &\XSolidBrush     &27.99 &0.732 &28.42 &0.711 \\
%     %                             &\Checkmark   &27.83 &0.726 &28.47 &0.705 \\
%     % \midrule
%     % \multirow{2}{*}{$\times 4$} &\XSolidBrush    &27.99 &0.730 &28.30 &0.704 \\
%     %                             &\Checkmark   &27.83 &0.729 &28.48 &0.702 \\
%     % \Xhline{1.5pt}
%     \end{tabular}
%     \end{adjustbox}
% % \end{footnotesize}
% \vspace{-1.0em}
% \end{table}


% \begin{table}
%     \centering
%     \caption{The ablation study of different proposed modules.  \textbf{(a)} The base model MiniGPT-4~\cite{zhu2023minigpt}. \textbf{(b)} The base model with ST-Adapter to capture the temporal cues. \textbf{(c)} MV-MLLM (Section~\ref{sec:baseline}) enhancing (b) with MV information. \textbf{(d)} Incorporating BEV into (b) for spatial cues. \textbf{(e)} BEV-InMLLM (Section~\ref{sec:bev-inmllm}) capturing all informations.}
%     \vspace{-3.0mm}
%     \label{tab:rgr_with_and_without_artifacts}
%     \begin{adjustbox}{max width=\linewidth}
%     \begin{tabular}{c|ccc|cc|cc|cc|c}
%     \Xhline{1.5pt}
%     \rowcolor{mygray}
%     &
%     &
%     &
%     &\multicolumn{2}{c|}{\it \textbf{Temporal}}
%     &\multicolumn{2}{c|}{\it \textbf{Multi-view}}
%     &\multicolumn{2}{c|}{\it \textbf{Spatial}}
%     &
%     \\
%     \rowcolor{mygray}
%      \multirow{-2}{*}{ \textbf{Model}}
%     &\multirow{-2}{*}{ \textbf{T}} 
%     &\multirow{-2}{*}{ \textbf{MV}}
%     &\multirow{-2}{*}{ \textbf{BEV}}
%     &\textbf{$\downarrow$}
%     &\textbf{$\uparrow$}
%      &\textbf{$\downarrow$}
%     &\textbf{$\uparrow$}
%    &\textbf{$\downarrow$}
%     &\textbf{$\uparrow$}
%     & \multirow{-2}{*}{\it \textbf{Whole} $\uparrow$}\\
%     % \cmidrule{1-1} \cmidrule{3-3} \cmidrule{5-5} \cmidrule{7-9} \cmidrule{11-15}
%   \midrule
%     \textbf{(a)}  & \XSolidBrush & \XSolidBrush  &  \XSolidBrush & 10.3 & 25.8 & 6.7 & 22.7 & 20.8 & 27.6 & 12.4  \\
%     \midrule
%  \multirow{2}{*}{\textbf{(b)}}  & \multirow{2}{*}{\Checkmark} & \XSolidBrush  &  \XSolidBrush &  7.4 & 28.5 &6.3 & 24.2 & 19.5 & 25.7 & 15.7 \\
%      \textbf{(c)}  &\Checkmark& \Checkmark &  \XSolidBrush &  6.4 & 31.4 & 4.1 & 30.7 & 18.0 &30.0 & 20.1\\
%      \textbf{(d)} & \Checkmark & \XSolidBrush  &  \Checkmark & 5.9 & 31.2 & 6.0 & 28.3 & 14.4 & 32.5 & 21.6  \\
%      \midrule
%      \textbf{(e)}  & \Checkmark & \Checkmark &  \Checkmark & 3.7 & 32.8 & 3.8 & 31.5 &13.9&32.9 & 22.2  \\
%   \bottomrule
%     % \multirow{2}{*}{$\times 2$} &\XSolidBrush    &28.16 &0.728 &28.08 &0.702 \\
%     %                             &\Checkmark   &27.99 &0.725 &28.05 &0.692 \\

%     % \midrule
%     % \multirow{2}{*}{$\times 3$} &\XSolidBrush     &27.99 &0.732 &28.42 &0.711 \\
%     %                             &\Checkmark   &27.83 &0.726 &28.47 &0.705 \\
%     % \midrule
%     % \multirow{2}{*}{$\times 4$} &\XSolidBrush    &27.99 &0.730 &28.30 &0.704 \\
%     %                             &\Checkmark   &27.83 &0.729 &28.48 &0.702 \\
%     % \Xhline{1.5pt}
%     \end{tabular}
%     \end{adjustbox}
% % \end{footnotesize}
% \vspace{-1.0em}
% \end{table}

==> sec/0_abstract.tex <==
\begin{abstract}
% As a key ingredient in autonomous driving, 
% Risk Object Localization and Intention Prediction (ROLISP) aims to identify, explain and localize the risk object for the ego-vehicle meanwhile predicting its intention, which has attracted increasing attention in autonomous driving field.
%
% In this paper, for the first time, we explore the potential of multimodal large language models (MLLMs) in the autonomous driving domain, focusing on the Risk Object Localization and Intention and Suggestion Prediction (ROLISP) task. 
% %
% ROLISP aims to identify, localize, and interpret risk objects for an ego-vehicle, simultaneously recognizing its intentions and providing motion suggestions.
% %
% However, when directly applied to the ROLISP task, present MLLMs usually face two main challenges,~\ie, failure detection of small objects (~\eg, traffic cones) and over-attention of salient objects (~\eg, large trucks).
% %
% To address the above problems, we present HiLM-D (\textbf{P}romote \textbf{P}erception \textbf{a}bility of ML\textbf{LM}s for Autonomous \textbf{Driv}ing), an efficient approach that leverages the vast knowledge stored in MLLMs, while tailoring it for the ROLISP task. 
Autonomous driving systems generally employ separate models for different tasks resulting in intricate designs.
%
For the first time, we leverage singular multimodal large language models (MLLMs) to consolidate multiple autonomous driving tasks from videos,~\ie, the Risk Object Localization and Intention and Suggestion Prediction (ROLISP) task.
%
ROLISP uses natural language to simultaneously identify and interpret risk objects, understand ego-vehicle intentions, and provide motion suggestions, eliminating the necessity for task-specific architectures.
%
However, lacking high-resolution (HR) information, existing MLLMs often miss small objects (\eg, traffic cones) and overly focus on salient ones (\eg, large trucks) when applied to ROLISP.
%
We propose HiLM-D (Towards \textbf{Hi}gh-Resolution Understanding in ML\textbf{LM}s for Autonomous \textbf{D}riving), an efficient method to incorporate HR information into MLLMs for the ROLISP task. 
%
Especially, HiLM-D integrates two branches: 
(i) the low-resolution reasoning branch, can be any MLLMs, processes low-resolution videos to caption risk objects and discern ego-vehicle intentions/suggestions; 
%
(ii) the high-resolution perception branch (HR-PB), prominent to HiLM-D, ingests HR images to enhance detection by capturing vision-specific HR feature maps and prioritizing all potential risks over merely salient objects.
%
Our HR-PB serves as a plug-and-play module, seamlessly fitting into current MLLMs. Experiments on the ROLISP benchmark reveal HiLM-D's notable advantage over leading MLLMs, with improvements of $4.8\%$ in BLEU-4 for captioning and $17.2\%$ in mIoU for detection.

% ROLISP aims to use the natural language as a unified output to identify, localize, and crack risk objects for an ego-vehicle, simultaneously recognizing its intentions and providing motion suggestions.
% (\eg, perception, reasoning, and prediction) using the natural captions, eliminating the necessity for task-specific architectures.
% introduce ROLISP to consolidate multi-tasks (\eg, perception, reasoning, and prediction) using the natural language produced by singular multimodal large language models (MLLMs), eliminating the necessity for task-specific architectures.
%
%
% ROLISP targets the identification, localization, and interpretation of risk objects for an ego-vehicle, while discerning its intentions and suggesting motions using the natural language paradigm. 
%
% investigates the capabilities of multimodal large language models (MLLMs) in autonomous driving, specifically for the Risk Object Localization and Intention and Suggestion Prediction (ROLISP) task.
%
% To address the above problems, we present HiLM-D (\textbf{P}romote \textbf{P}erception \textbf{a}bility of ML\textbf{LM}s for Autonomous \textbf{Driv}ing), an efficient approach that leverages the vast knowledge stored in MLLMs, while tailoring it for the ROLISP task. 
% %
% Specially, HiLM-D consists of two branches: a low resolution reasoning branch (LR-RB) and a a high resolution perception branch (HR-PB).
% %
% LR-RB, can be any MLLM, ingests low resolution videos to caption risk objects and infer ego-vehicle intentions/suggestions.
% %
% HR-PB, the key component of HiLM-D, receives high resolution (HR) image to: (i) capture HR feature maps with vision-specific prior thus improving detection accuracy; (ii) focus on all potential risk objects instead of only salient objects, boosting risk object identification accuracy.
% \if
% We propose HiLM-D (\textbf{P}romote \textbf{P}erception \textbf{a}bility of ML\textbf{LM}s for Autonomous \textbf{Driv}ing), a method harnessing MLLMs' extensive knowledge, tailored for the ROLISP task. 
% %
% Specially, HiLM-D integrates two branches: 
% (i) the low-resolution reasoning branch, can be any MLLMs, processes low-resolution videos to caption risk objects and discern ego-vehicle intentions/suggestions; 
% %
% (ii) the high-resolution perception branch (HR-PB), prominent to HiLM-D, ingests high-resolution images to enhance detection by capturing vision-specific HR feature maps and prioritizing all potential risks over merely salient objects.
% Specially, HiLM-D incorporates the high-resolution feature maps with vision-specific prior knowledge into the MLLMs to promote the detection performance by a parameter-efficient and computation-friend way.
%
% LR-RB, can be any MLLMs, aims to receive the low resolution (LR) videos as input and generate the caption for the risk object with explanations and ego-vehicle intention/suggestion.
%
% Moreover, HiLM-D utilizes an enumeration module to focus on all potential risk objects instead of only salient objects, boosting risk object identification accuracy.
% Note that our HR-PB is a plug-and-play module that can be easily integrated into existing MLLMs.
% %
% Comprehensive experiment results on the ROLISP benchmark demonstrate the superiority of HiLM-D over the state-of-the-art MLLMs, e.g., by $4.8\%$ on BLEU-4 and $17.2\%$ on mIoU.
%
% Our HR-PB serves as a plug-and-play module, seamlessly fitting into current MLLMs. Experiments on the ROLISP benchmark reveal HiLM-D's notable advantage over leading MLLMs, with improvements of $4.8\%$ in BLEU-4 for captioning and $17.2\%$ in mIoU for detection.





%------------------------------
% \if
% In this paper, for the first time, we explore the reasoning ability of multimodal large language models (MLLMs) for an autonomous driving task,~\ie, Risk Object Localization and Intention and Suggestion Prediction (ROLISP) that aims to identify, explain and localize the risk object for the ego-vehicle meanwhile recognizing its intention and giving the motion suggestions.
% %
% However, when applying to ROLISP, current MLLMs face two main problems,~\ie, failure detection of small objects (~\eg, traffic cones) and over-attention of salient objects (~\eg, large trucks).
% %
% To address the above problems, we present P$^2$alm Drive (\textbf{P}romote \textbf{P}erception \textbf{a}bility of ML\textbf{LM}s for Autonomous Driving), an efficient approach that leverages the vast knowledge stored in MLLMs, while tailoring it for ROLISP task. 
% %
% To address the above problems, we propose a simple yet efficient method to \textbf{P}r\textbf{O}mote the \textbf{P}erception ability of \textbf{M}LLMs for \textbf{A}utonomous \textbf{D}riving named POPMAD.
% %
% % Considering the current 
% The proposed POPMAD incurs three advantages:
% (i) POPMAD is training-efficient due to leveraging the frozen pre-trained MLLM;
% %
% (ii) POPMAD incorporates the high-resolution feature maps with vision-specific prior knowledge into the MLLMs to promote the detection performance by a parameter-efficient and computation-friend way;
% %
% (iii) POPMAD use an enumeration module to focus on all potential risk objects instead of only salient objects, thus improving the accuracy of risk object identification;
% %
% (iv) POPMAD is a plug-and-play module that can be easily integrated into existing MLLMs.
% % Inspired by the remarkable reasoning ability of recent multimodal large language models (MLLMs), we 
% Extensive experiments demonstrate that POPMAD outperforms current state-of-the-art MLLMs on the ROLISP benchmark.
% \fi

% \if
% \hjh{In this paper, for the first time, we explore the potential of multimodal large-language-models (MLLMs) in the autonomous driving domain, with a focus on the Risk Object Localization and Intention and Suggestion Prediction (ROLISP) task. 
% ROLISP aims to detect, localize, and interpret risk objects for an ego-vehicle, simultaneously recognizing their intentions and providing the motion suggestions.
% However, when directly applied into ROLISP task, present MLLMs usually struggle with detecting smaller objects (~\eg, traffic cones) and tend to overly focus on conspicuous items (~\eg, large trucks). 
% To address the above problems, 
% we present POPMAD (Promote Perception ability of MLLMs for Autonomous Driving), an efficient approach that leverage the vast knowledge stored in MLLMs, while tailoring it for ROLISP task. 
% Specially, 
% POPMAD incorporates the high-resolution feature maps with vision-specific prior knowledge into the MLLMs to promote the detection performance by a parameter-efficient and computation-friend way.
% Moreover, POPMAD utilize an enumeration module to focus on all potential risk objects instead of only salient objects, boosting risk object identification accuracy.
% Note that our POPMAD is a plug-and-play module that can be easily integrated into existing MLLMs.
% Comprehensive experiment results on ROLISP benchmark demonstrate the POPMAD's superiority over the state-of-the-art MLLMs, e.g., XXX.}
% \fi
\end{abstract}

==> sec/1_intro.tex <==
\section{Introduction}
\label{sec:intro}

Please follow the steps outlined below when submitting your manuscript to the IEEE Computer Society Press.
This style guide now has several important modifications (for example, you are no longer warned against the use of sticky tape to attach your artwork to the paper), so all authors should read this new version.

%-------------------------------------------------------------------------
\subsection{Language}

All manuscripts must be in English.

\subsection{Dual submission}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a
discussion of the policy on dual submissions.

\subsection{Paper length}
Papers, excluding the references section, must be no longer than eight pages in length.
The references section will not be included in the page count, and there is no limit on the length of the references section.
For example, a paper of eight pages with two pages of references would have a total length of 10 pages.
{\bf There will be no extra page charges for \confName\ \confYear.}

Overlength papers will simply not be reviewed.
This includes papers where the margins and formatting are deemed to have been significantly altered from those laid down by this style guide.
Note that this \LaTeX\ guide already sets figure captions and references in a smaller font.
The reason such papers will not be reviewed is that there is no provision for supervised revisions of manuscripts.
The reviewing process cannot determine the suitability of the paper for presentation in eight pages if it is reviewed in eleven.

%-------------------------------------------------------------------------
\subsection{The ruler}
The \LaTeX\ style defines a printed ruler which should be present in the version submitted for review.
The ruler is provided in order that reviewers may comment on particular lines in the paper without circumlocution.
If you are preparing a document using a non-\LaTeX\ document preparation system, please arrange for an equivalent ruler to appear on the final output pages.
The presence or absence of the ruler should not change the appearance of any other content on the page.
The camera-ready copy should not contain a ruler.
(\LaTeX\ users may use options of \texttt{cvpr.sty} to switch between different versions.)

Reviewers:
note that the ruler measurements do not align well with lines in the paper --- this turns out to be very difficult to do well when the paper contains many figures and equations, and, when done, looks ugly.
Just use fractional references (\eg, this line is $087.5$), although in most cases one would expect that the approximate location will be adequate.


\subsection{Paper ID}
Make sure that the Paper ID from the submission system is visible in the version submitted for review (replacing the ``*****'' you see in this document).
If you are using the \LaTeX\ template, \textbf{make sure to update paper ID in the appropriate place in the tex file}.


\subsection{Mathematics}

Please number all of your sections and displayed equations as in these examples:
\begin{equation}
  E = m\cdot c^2
  \label{eq:important}
\end{equation}
and
\begin{equation}
  v = a\cdot t.
  \label{eq:also-important}
\end{equation}
It is important for readers to be able to refer to any particular equation.
Just because you did not refer to it in the text does not mean some future reader might not need to refer to it.
It is cumbersome to have to use circumlocutions like ``the equation second from the top of page 3 column 1''.
(Note that the ruler will not be present in the final copy, so is not an alternative to equation numbers).
All authors will benefit from reading Mermin's description of how to write mathematics:
\url{http://www.pamitc.org/documents/mermin.pdf}.

\subsection{Blind review}

Many authors misunderstand the concept of anonymizing for blind review.
Blind review does not mean that one must remove citations to one's own work---in fact it is often impossible to review a paper unless the previous citations are known and available.

Blind review means that you do not use the words ``my'' or ``our'' when citing previous work.
That is all.
(But see below for tech reports.)

Saying ``this builds on the work of Lucy Smith [1]'' does not say that you are Lucy Smith;
it says that you are building on her work.
If you are Smith and Jones, do not say ``as we show in [7]'', say ``as Smith and Jones show in [7]'' and at the end of the paper, include reference 7 as you would any other cited work.

An example of a bad paper just asking to be rejected:
\begin{quote}
\begin{center}
    An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of our previous paper [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Removed for blind review
\end{quote}


An example of an acceptable paper:
\begin{quote}
\begin{center}
     An analysis of the frobnicatable foo filter.
\end{center}

   In this paper we present a performance analysis of the  paper of Smith \etal [1], and show it to be inferior to all previously known methods.
   Why the previous paper was accepted without this analysis is beyond me.

   [1] Smith, L and Jones, C. ``The frobnicatable foo filter, a fundamental contribution to human knowledge''. Nature 381(12), 1-213.
\end{quote}

If you are making a submission to another conference at the same time, which covers similar or overlapping material, you may need to refer to that submission in order to explain the differences, just as you would if you had previously published related work.
In such cases, include the anonymized parallel submission~\cite{Authors14} as supplemental material and cite it as
\begin{quote}
[1] Authors. ``The frobnicatable foo filter'', F\&G 2014 Submission ID 324, Supplied as supplemental material {\tt fg324.pdf}.
\end{quote}

Finally, you may feel you need to tell the reader that more details can be found elsewhere, and refer them to a technical report.
For conference submissions, the paper must stand on its own, and not {\em require} the reviewer to go to a tech report for further details.
Thus, you may say in the body of the paper ``further details may be found in~\cite{Authors14b}''.
Then submit the tech report as supplemental material.
Again, you may not assume the reviewers will read this material.

Sometimes your paper is about a problem which you tested using a tool that is widely known to be restricted to a single institution.
For example, let's say it's 1969, you have solved a key problem on the Apollo lander, and you believe that the 1970 audience would like to hear about your
solution.
The work is a development of your celebrated 1968 paper entitled ``Zero-g frobnication: How being the only people in the world with access to the Apollo lander source code makes us a wow at parties'', by Zeus \etal.

You can handle this paper like any other.
Do not write ``We show how to improve our previous work [Anonymous, 1968].
This time we tested the algorithm on a lunar lander [name of lander removed for blind review]''.
That would be silly, and would immediately identify the authors.
Instead write the following:
\begin{quotation}
\noindent
   We describe a system for zero-g frobnication.
   This system is new because it handles the following cases:
   A, B.  Previous systems [Zeus et al. 1968] did not  handle case B properly.
   Ours handles it by including a foo term in the bar integral.

   ...

   The proposed system was integrated with the Apollo lunar lander, and went all the way to the moon, don't you know.
   It displayed the following behaviours, which show how well we solved cases A and B: ...
\end{quotation}
As you can see, the above text follows standard scientific convention, reads better than the first version, and does not explicitly name you as the authors.
A reviewer might think it likely that the new paper was written by Zeus \etal, but cannot make any decision based on that guess.
He or she would have to be sure that no other authors could have been contracted to solve problem B.
\medskip

\noindent
FAQ\medskip\\
{\bf Q:} Are acknowledgements OK?\\
{\bf A:} No.  Leave them for the final copy.\medskip\\
{\bf Q:} How do I cite my results reported in open challenges?
{\bf A:} To conform with the double-blind review policy, you can report results of other challenge participants together with your results in your paper.
For your results, however, you should not identify yourself and should not mention your participation in the challenge.
Instead present your results referring to the method proposed in your paper and draw conclusions based on the experimental comparison to other results.\medskip\\

\begin{figure}[t]
  \centering
  \fbox{\rule{0pt}{2in} \rule{0.9\linewidth}{0pt}}
   %\includegraphics[width=0.8\linewidth]{egfigure.eps}

   \caption{Example of caption.
   It is set in Roman so that mathematics (always set in Roman: $B \sin A = A \sin B$) may be included without an ugly clash.}
   \label{fig:onecol}
\end{figure}

\subsection{Miscellaneous}

\noindent
Compare the following:\\
\begin{tabular}{ll}
 \verb'$conf_a$' &  $conf_a$ \\
 \verb'$\mathit{conf}_a$' & $\mathit{conf}_a$
\end{tabular}\\
See The \TeX book, p165.

The space after \eg, meaning ``for example'', should not be a sentence-ending space.
So \eg is correct, {\em e.g.} is not.
The provided \verb'\eg' macro takes care of this.

When citing a multi-author paper, you may save space by using ``et alia'', shortened to ``\etal'' (not ``{\em et.\ al.}'' as ``{\em et}'' is a complete word).
If you use the \verb'\etal' macro provided, then you need not worry about double periods when used at the end of a sentence as in Alpher \etal.
However, use it only when there are three or more authors.
Thus, the following is correct:
   ``Frobnication has been trendy lately.
   It was introduced by Alpher~\cite{Alpher02}, and subsequently developed by
   Alpher and Fotheringham-Smythe~\cite{Alpher03}, and Alpher \etal~\cite{Alpher04}.''

This is incorrect: ``... subsequently developed by Alpher \etal~\cite{Alpher03} ...'' because reference~\cite{Alpher03} has just two authors.

\begin{figure*}
  \centering
  \begin{subfigure}{0.68\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{An example of a subfigure.}
    \label{fig:short-a}
  \end{subfigure}
  \hfill
  \begin{subfigure}{0.28\linewidth}
    \fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
    \caption{Another example of a subfigure.}
    \label{fig:short-b}
  \end{subfigure}
  \caption{Example of a short caption, which should be centered.}
  \label{fig:short}
\end{figure*}


==> sec/2_formatting.tex <==
\section{Formatting your paper}
\label{sec:formatting}

All text must be in a two-column format.
The total allowable size of the text area is $6\frac78$ inches (17.46 cm) wide by $8\frac78$ inches (22.54 cm) high.
Columns are to be $3\frac14$ inches (8.25 cm) wide, with a $\frac{5}{16}$ inch (0.8 cm) space between them.
The main title (on the first page) should begin 1 inch (2.54 cm) from the top edge of the page.
The second and following pages should begin 1 inch (2.54 cm) from the top edge.
On all pages, the bottom margin should be $1\frac{1}{8}$ inches (2.86 cm) from the bottom edge of the page for $8.5 \times 11$-inch paper;
for A4 paper, approximately $1\frac{5}{8}$ inches (4.13 cm) from the bottom edge of the
page.

%-------------------------------------------------------------------------
\subsection{Margins and page numbering}

All printed material, including text, illustrations, and charts, must be kept
within a print area $6\frac{7}{8}$ inches (17.46 cm) wide by $8\frac{7}{8}$ inches (22.54 cm)
high.
%
Page numbers should be in the footer, centered and $\frac{3}{4}$ inches from the bottom of the page.
The review version should have page numbers, yet the final version submitted as camera ready should not show any page numbers.
The \LaTeX\ template takes care of this when used properly.



%-------------------------------------------------------------------------
\subsection{Type style and fonts}

Wherever Times is specified, Times Roman may also be used.
If neither is available on your word processor, please use the font closest in
appearance to Times to which you have access.

MAIN TITLE.
Center the title $1\frac{3}{8}$ inches (3.49 cm) from the top edge of the first page.
The title should be in Times 14-point, boldface type.
Capitalize the first letter of nouns, pronouns, verbs, adjectives, and adverbs;
do not capitalize articles, coordinate conjunctions, or prepositions (unless the title begins with such a word).
Leave two blank lines after the title.

AUTHOR NAME(s) and AFFILIATION(s) are to be centered beneath the title
and printed in Times 12-point, non-boldface type.
This information is to be followed by two blank lines.

The ABSTRACT and MAIN TEXT are to be in a two-column format.

MAIN TEXT.
Type main text in 10-point Times, single-spaced.
Do NOT use double-spacing.
All paragraphs should be indented 1 pica (approx.~$\frac{1}{6}$ inch or 0.422 cm).
Make sure your text is fully justified---that is, flush left and flush right.
Please do not place any additional blank lines between paragraphs.

Figure and table captions should be 9-point Roman type as in \cref{fig:onecol,fig:short}.
Short captions should be centred.

\noindent Callouts should be 9-point Helvetica, non-boldface type.
Initially capitalize only the first word of section titles and first-, second-, and third-order headings.

FIRST-ORDER HEADINGS.
(For example, {\large \bf 1. Introduction}) should be Times 12-point boldface, initially capitalized, flush left, with one blank line before, and one blank line after.

SECOND-ORDER HEADINGS.
(For example, { \bf 1.1. Database elements}) should be Times 11-point boldface, initially capitalized, flush left, with one blank line before, and one after.
If you require a third-order heading (we discourage it), use 10-point Times, boldface, initially capitalized, flush left, preceded by one blank line, followed by a period and your text on the same line.

%-------------------------------------------------------------------------
\subsection{Footnotes}

Please use footnotes\footnote{This is what a footnote looks like.
It often distracts the reader from the main flow of the argument.} sparingly.
Indeed, try to avoid footnotes altogether and include necessary peripheral observations in the text (within parentheses, if you prefer, as in this sentence).
If you wish to use a footnote, place it at the bottom of the column on the page on which it is referenced.
Use Times 8-point type, single-spaced.


%-------------------------------------------------------------------------
\subsection{Cross-references}

For the benefit of author(s) and readers, please use the
{\small\begin{verbatim}
  \cref{...}
\end{verbatim}}  command for cross-referencing to figures, tables, equations, or sections.
This will automatically insert the appropriate label alongside the cross-reference as in this example:
\begin{quotation}
  To see how our method outperforms previous work, please see \cref{fig:onecol} and \cref{tab:example}.
  It is also possible to refer to multiple targets as once, \eg~to \cref{fig:onecol,fig:short-a}.
  You may also return to \cref{sec:formatting} or look at \cref{eq:also-important}.
\end{quotation}
If you do not wish to abbreviate the label, for example at the beginning of the sentence, you can use the
{\small\begin{verbatim}
  \Cref{...}
\end{verbatim}}
command. Here is an example:
\begin{quotation}
  \Cref{fig:onecol} is also quite important.
\end{quotation}

%-------------------------------------------------------------------------
\subsection{References}

List and number all bibliographical references in 9-point Times, single-spaced, at the end of your paper.
When referenced in the text, enclose the citation number in square brackets, for
example~\cite{Authors14}.
Where appropriate, include page numbers and the name(s) of editors of referenced books.
When you cite multiple papers at once, please make sure that you cite them in numerical order like this \cite{Alpher02,Alpher03,Alpher05,Authors14b,Authors14}.
If you use the template as advised, this will be taken care of automatically.

\begin{table}
  \centering
  \begin{tabular}{@{}lc@{}}
    \toprule
    Method & Frobnability \\
    \midrule
    Theirs & Frumpy \\
    Yours & Frobbly \\
    Ours & Makes one's heart Frob\\
    \bottomrule
  \end{tabular}
  \caption{Results.   Ours is better.}
  \label{tab:example}
\end{table}

%-------------------------------------------------------------------------
\subsection{Illustrations, graphs, and photographs}

All graphics should be centered.
In \LaTeX, avoid using the \texttt{center} environment for this purpose, as this adds potentially unwanted whitespace.
Instead use
{\small\begin{verbatim}
  \centering
\end{verbatim}}
at the beginning of your figure.
Please ensure that any point you wish to make is resolvable in a printed copy of the paper.
Resize fonts in figures to match the font in the body text, and choose line widths that render effectively in print.
Readers (and reviewers), even of an electronic copy, may choose to print your paper in order to read it.
You cannot insist that they do otherwise, and therefore must not assume that they can zoom in to see tiny details on a graphic.

When placing figures in \LaTeX, it's almost always best to use \verb+\includegraphics+, and to specify the figure width as a multiple of the line width as in the example below
{\small\begin{verbatim}
   \usepackage{graphicx} ...
   \includegraphics[width=0.8\linewidth]
                   {myfile.pdf}
\end{verbatim}
}


%-------------------------------------------------------------------------
\subsection{Color}

Please refer to the author guidelines on the \confName\ \confYear\ web page for a discussion of the use of color in your document.

If you use color in your plots, please keep in mind that a significant subset of reviewers and readers may have a color vision deficiency; red-green blindness is the most frequent kind.
Hence avoid relying only on color as the discriminative feature in plots (such as red \vs green lines), but add a second discriminative feature to ease disambiguation.

==> sec/3_finalcopy.tex <==
\section{Final copy}

You must include your signed IEEE copyright release form when you submit your finished paper.
We MUST have this form before your paper can be published in the proceedings.

Please direct any questions to the production editor in charge of these proceedings at the IEEE Computer Society Press:
\url{https://www.computer.org/about/contact}.
